Fermi surface evolution and checker-board block-spin antiferromagnetism in $A_x$Fe$_{2-y}$Se$_{2}$

We develop an effective multiorbital mean-field t-J Hamiltonian with realistic tight-binding and exchange parameters to describe the electronic and magnetic structures of iron-selenide based superconductors $A_x$Fe$_{2-y}$Se$_2$ for iron vacancy doping in the range $0 \leq y \leq 0.4$. The Fermi surface topology extracted from the spectral function of angle-resolved photoemission spectroscopy (ARPES) experiments is adequately accounted for by a tight-binding lattice model with random vacancy disorder. Since introducing iron vacancies breaks the lattice periodicity of the stochiometric compound, it greatly affects the electronic band structure. With changing vacancy concentration the electronic band structure evolves, leading to a reconstruction of the Fermi surface topology. For intermediate doping levels, the realized stable electronic structure is a compromise between the solutions for the perfect lattice with $y=0$ and the vacancy stripe-ordered lattice with $y=0.4$, which results in a competition between vacancy random disorder and vacancy stripe order. A multiorbital hopping model is parameterized by fitting Fermi surface topologies to ARPES experiments, from which we construct a mean-field t-J lattice model to study the paramagnetic and antiferromagnetic (AFM) phases of K$_{0.8}$Fe$_{1.6}$Se$_2$. In the AFM phase the calculated spin magnetization of the t-J model leads to a checker-board block-spin structure in good agreement with neutron scattering experiments and {\it ab}-{\it initio} calculations.

==> my_tools.tex <==
%------------------------------------------------------------------------------------
%% Switch for the definition of pages.
\newcommand{\PAGE}	[1]	{
%	{\normalsize \colorbox{red}{#1}}
}
%------------------------------------------------------------------------------------
%% Switch for the includegraphics which show the pictures.
\newcommand{\Ig}[2]{
		\includegraphics[width=#1]{#2}
}
%------------------------------------------------------------------------------------

\newcommand{\Fig}	[3] {
	\begin{figure}[htbp] 
	\centering 
	\Ig{#1}{#2} 
	\caption[]{#3} 
	\end{figure} 
}
\newcommand{\Figs}	[2] {
	\begin{figure}[htbp] 
	\centering 
	#1
	\caption[]{#2} 
	\end{figure} 
}
\newcommand{\EqFig}		[2]{ 
		\Align{\mbox{\Ig{#1}{#2}}
%		\\ \mbox{\small #2 }
} }
\newcommand{\EqFigT}		[3]{ 
		\Gather{\mbox{\Ig{#1}{#2}}
		\\ \mbox{\small #3 }
} }
\newcommand{\EqFigBr}	[2]{ \bigg( \Align{ \mbox{\Ig{#1}{#2}} }\bigg) }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Some simplified tems which may be used mostly
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\T}				{\,T\; }
\newcommand{\ab}			{{\alpha\beta}}
\newcommand{\Tt}			{\,T_\tau\, }
\newcommand{\Piab}			{\Pi_{\alpha\beta} }
\newcommand{\hV}			{\,\hat V}
\newcommand{\hA}			{\,\hat A}
\newcommand{\hvec}		[1]	{\,\hat{\vec #1}}
\newcommand{\dv}		[1]	{\,\dot{\vec #1}}
\newcommand{\ddv}		[1]	{\,\ddot{\vec #1}}
\newcommand{\ds}			{\displaystyle}
\newcommand{\C}			[1]	{\,C_{#1}}
\newcommand{\Cd}		[1]	{\,C^\dagger_{#1}}
\newcommand{\Cdp}		[1]	{\,C^{'\dagger}_{#1}}
\newcommand{\ad}		[1]	{\,a_{#1}^\dagger}
\newcommand{\hC}		[1]	{\,\hat C_{#1}}
\newcommand{\hCd}		[1]	{\,\hat C_{#1}^\dagger}
\newcommand{\Gz}			{\,G^{(0)}}
\newcommand{\mG}			{\mathcal{G} }
\newcommand{\mGz}			{\,\mathcal{G}^{(0)}}
\newcommand{\Dz}			{\,D^{(0)}}
\newcommand{\mD}			{\mathcal{D} }
\newcommand{\mDz}			{\,\mathcal{D}^{(0)}}
\newcommand{\Po}			{P^{(1)}}
\newcommand{\Sig}		[1]	{\,\Sigma^{(#1)}}
\newcommand{\Pii}		[1]	{\,\Pi^{(#1)}}
\newcommand{\Sigo}			{\,\Sigma^{(1)}}
\newcommand{\Sigf}			{\,\Sigma^{(F)}}
\newcommand{\Sigh}			{\,\Sigma^{(H)}}
\newcommand{\Sighp}			{\,\Sigma^{(H)'}}
\newcommand{\vp}			{\vec p}
\newcommand{\vpp}			{\vec p'}
\newcommand{\vppp}			{\vec p''}
\newcommand{\vk}			{\vec k}
\newcommand{\vq}			{\vec q}
\newcommand{\vqp}			{\vec {q'}}
\newcommand{\intff}			{\int_{-\infty}^\infty}
\newcommand{\intzb}			{\int_0^\beta}
\newcommand{\intzp}			{\int_0^\pi}
\newcommand{\intpz}			{\int_\pi^0}
\newcommand{\intztp}			{\int_0^{2\pi}}
\newcommand{\intzf}			{\int_0^\infty}
\newcommand{\intfz}			{\int_{-\infty}^0}
\newcommand{\intzt}			{\int_0^t}
\newcommand{\intft}			{\int_{-\infty}^t}
\newcommand{\ppartial}	[2]	{\frac{\partial #1}{\partial #2}}
\newcommand{\ssum}		[1]	{\sum_{\substack{#1}}}
\newcommand{\dd}		[1]	{\frac{d}{d#1}}
\newcommand{\Res}			{\mbox{Res}}
\newcommand{\Ery}			{E_{Ry}}
\newcommand{\Sign}			{\;\mbox{Sign}}
\newcommand{\Sy}{ S(y) = -\bigg(1+{1-y^2\over 2y}\ln|{1+y\over 1-y}|\bigg) }
\newcommand{\OO}			{\over}

\newcommand{\vkq}			{{\vk+\vq}}
\newcommand{\vkqp}			{{\vk+\vqp}}
\newcommand{\vkqq}			{{\vk+\vq+\vqp}}

\newcommand{\vpq}			{{\vp+\vq}}
\newcommand{\vpqp}			{{\vp+\vqp}}
\newcommand{\vpqq}			{{\vp+\vq+\vqp}}

\newcommand{\xkq}			{\xi_{\vk+\vq}}
\newcommand{\xkqp}			{\xi_{\vk+\vqp}}
\newcommand{\xkqq}			{\xi_{\vk+\vq+\vqp}}
\newcommand{\iwnm}			{iw_n + iw_m}

\newcommand{\atan}			{\tan^{-1}}
\newcommand{\im}			{\;\mathcal{I}m\,}
%\newcommand{\re}			{\;\mathcal{R}e\,}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\Align}		[1]	{\begin{aligned} #1 \end{aligned}}
\newcommand{\Gather}	[1]	{\begin{gathered} #1 \end{gathered}}
\newcommand{\Split}		[1]	{\begin{split} #1 \end{split}}

\newcommand{\Cases}		[1]	{ \begin{cases} #1 \end{cases} }
\newcommand{\CasesAlign}[1]	{ \Align{\begin{cases} #1 \end{cases}} }

\newcommand{\Eq}		[1]	{\begin{equation*} #1 \end{equation*}}
\newcommand{\Eqn}		[1]	{\begin{equation} #1 \end{equation}}
\newcommand{\Eqs}		[1]	{\begin{subequations} #1 \end{subequations}}

\newcommand{\EqGather}	[1]	{\begin{gather*} #1 \end{gather*}}
\newcommand{\EqnGather}	[1]	{\Eqn{ \Gather{ #1}}}
\newcommand{\EqnnGather}[1]	{\begin{gather} #1 \end{gather}}
\newcommand{\EqsGather}	[2]	{\begin{subequations}\label{#1} \begin{gather} #2 \end{gather} \end{subequations}}

\newcommand{\EqAlign}	[1]	{\begin{align*} #1 \end{align*}}
\newcommand{\EqnAlign}	[1]	{\Eqn{ \Align{ #1}}}			%For single line description
\newcommand{\EqnnAlign}	[1]	{\begin{align} #1 \end{align}}	%For multiple line description
\newcommand{\EqsAlign}	[2]	{\begin{subequations} \label{#1} \begin{align} #2 \end{align} \end{subequations}}


%%%%%%%%%%%%%%%%%%%%%%% Enumerate %%%%%%%%%%%%%%%%%
\newcommand{\Enumerate}	[1]	{\begin{enumerate} #1 \end{enumerate}}
\newcommand{\Itemize}	[1]	{\begin{itemize} #1 \end{itemize}}			%For single line description
\newcommand{\Description}[1]{\begin{description} #1 \end{description}}	%For multiple line description
%%%%%%%%%%%%%%%%%%%%%%% Enumerate %%%%%%%%%%%%%%%%%

\newcommand{\Tr}		[1]	{\mbox{Tr}\big[\, #1 \, \big]}
\newcommand{\fTr}		[2]	{ \frac{\Tr{#1}}{\Tr{#2}}}

\newcommand{\Bracket}	[1]	{\langle \, #1 \, \rangle}
\newcommand{\BK}		[1]	{\langle \, #1 \, \rangle}

%%%%%%%%%%%%%%%%%%%%%%% big %%%%%%%%%%%%%%%%
\newcommand{\bigBR}		[1]	{\big\{  #1\big\} }
\newcommand{\biggBR}	[1]	{\bigg\{ #1\bigg\}}
\newcommand{\BigBR}		[1]	{\big\{  #1\big\} }
\newcommand{\BiggBR}	[1]	{\bigg\{ #1\bigg\}}

\newcommand{\bigBB}		[1]	{\big[ {#1}\big]}
\newcommand{\biggBB}	[1]	{\bigg[{#1}\bigg]}
\newcommand{\BigBB}		[1]	{\big[ {#1}\big]}
\newcommand{\BiggBB}	[1]	{\bigg[{#1}\bigg]}

\newcommand{\bigBC}		[1]	{\big({#1}\big)}
\newcommand{\biggBC}	[1]	{\bigg({#1}\bigg)}
\newcommand{\BigBC}		[1]	{\big({#1}\big)}
\newcommand{\BiggBC}	[1]	{\bigg({#1}\bigg)}
%%%%%%%%%%%%%%%%%%%%%%% big %%%%%%%%%%%%%%%%

\newcommand{\zBracket}	[1]	{\,_0\langle \, #1 \, \rangle_0\,}
\newcommand{\zBK}		[1]	{\,_0\langle \, #1 \, \rangle_0\,}
\newcommand{\BraKat}	[2]	{\langle \, #1 \mid #2 \, \rangle}
\newcommand{\zBraKat}	[2]	{\,_0\langle \, #1 \mid #2 \, \rangle_0\,}
\newcommand{\Bra}		[1]	{\langle \,  #1  \mid}
\newcommand{\Kat}		[1]	{\mid  #1 \, \rangle}
\newcommand{\zBra}		[1]	{\,_0\langle \,  #1  \mid}
\newcommand{\zKat}		[1]	{\mid  #1 \, \rangle_0\,}

\newcommand{\Com} [1] {\;\big[ \; #1 \;\big]} %for the commutation relation

%%%%%%%%%%%%%%%%%%%%%%% Table %%%%%%%%%%%%%%%%%
\newcommand{\tab}	[2]	{
	\begin{tabular}{#1}
	\\
		#2
	\\ \\
	\end{tabular}
}

%%%%%%%%%%%%% Wick Contraction %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\wABCD}			[4]	{
	\contraction[2ex]{}{#1}{}{#2}
	\contraction[2ex]{#1#2}{#3}{}{#4}
	#1#2#3#4
}
\newcommand{\wACBD}			[4]	{
	\contraction{}{#1}{#2}{#3} 
	\bcontraction[2ex]{#1}{#2}{#3}{#4} 
	#1#2#3#4
}
\newcommand{\wADBC}			[4]	{
	\contraction{}{#1}{#2#3}{#4} 
	\bcontraction[2ex]{#1}{#2}{}{#3} 
	#1#2#3#4
}

%\newcommand{\wABCDEF}			[6]	{
%	\contraction[2ex]{}{#1}{}{#2}
%	\contraction[2ex]{#1#2}{#3}{}{#4}
%	\contraction[2ex]{#1#2#3#4}{#5}{}{#6}
%	#1#2#3#4
%}
%%%%%%%%%%%%%%%%%%%%%%%HOME WORK%%%%%%%%%%%%%%%%%
\newcommand{\HomeWork}	[1] { {\bf\large $\S$ Home work #1:}\quad}

\newcommand{\HomeWorkH}	[2] {
{\bf\large $\S$ Home work #1:} ------------------------------------------------------------------------------------------
\\#2
\EqGather{\hline}
}
%%%%%%%%%%%%%%%%%%%%%%%HOME WORK%%%%%%%%%%%%%%%%%











